Accurate, private, secure, federated U-statistics with higher degree

We study the problem of computing a U-statistic with a kernel function f of degree k $\ge$ 2, i.e., the average of some function f over all k-tuples of instances, in a federated learning setting. Ustatistics of degree 2 include several useful statistics such as Kendall's $\tau$ coefficient, the Area under the Receiver-Operator Curve and the Gini mean difference. Existing methods provide solutions only under the lower-utility local differential privacy model and/or scale poorly in the size of the domain discretization. In this work, we propose a protocol that securely computes U-statistics of degree k $\ge$ 2 under central differential privacy by leveraging Multi Party Computation (MPC). Our method substantially improves accuracy when compared to prior solutions. We provide a detailed theoretical analysis of its accuracy, communication and computational properties. We evaluate its performance empirically, obtaining favorable results, e.g., for Kendall's $\tau$ coefficient, our approach reduces the Mean Squared Error by up to four orders of magnitude over existing baselines.

==> tmp.tex <==


\section{Proposed protocol}

\subsection{Overview}

In a first phase called offline phase, parties exchange some correlated randomness 
in order to speed up the computation during the online phase (see subsection \ref{app:mpc_preproc}).
Also, some subset $E\subseteq \nkcombs^n_k $ 
is sampled inducing a sample of the set of all $k$-tuples $\comb{ \{ x_i \}_{i \in [n]} }{k}$.
The set $E$ defines a graph $G = (V, E)$, where $V$ denotes the set of vertices representing the parties and $E$ the edges connecting them. 
Then, during the online phase,
parties compute the incomplete U-statistic parametrized by the set of edges $E$.
Next, the parties generate and add shared noise $\eta$ sampled from the Laplace (resp. Gaussian) distribution, 
thereby ensuring that the outcome satisfies central $\epsilon$-DP (resp. $(\epsilon, \delta)$-DP).
The computations are done in the finite field $\mathbb{F}$.
% which represents the fractional numbers with a fixed number of decimals.
Let $\hat{U}_{f, E}$ denote our estimator of $U_{f, C^n_k}$.  
Our goal is to minimize the variance of $\hat{U}_{f, E}$ while minimizing the communication complexity. 

\subsection{More notations}

Let $G = (V, E)$ be a $k$-uniform hypergraph where $V = \{1, \dots, n\}$ is the set of vertices and $E = \{ ( {i_1}, \ldots, {i_k} ) \} \subseteq \comb{V}{k}$ is a set of hyperedges. 
A $G=(V, E)$ hypergraph is $k$-uniform if for all $e \in E$, $|e| = k$.
$V$ represents the parties while $E$ is the set of all $k$-tuples we evaluate $f$ on.
For a set $S$, let $E_{ S }$ be the set of edges in $E$ that contains $S$, i.e., $E_S = \{ e \in E: S \subseteq e \}$.
Let $p = \underset{i \in [n]}{\esp}[ | E_{ \{ i \}} |]$ be the expected number of neighbors per party.
Note that $p$ depends on the sampling method for $E \subseteq C^n_k$. 

\begin{figure}[ht]
  \begin{func}[Functionality $\mathcal{F}_f$]
    \textbf{Input}: Functionality $\mathcal{F}_f$ receives $(e, i_j, \mathcal{S}_{i_j})$ from party $P_{i_j}$ 
    for all parties $P_{i_1}, \ldots, P_{i_k}$ 
    where $e = (i_1, \ldots, i_k)$ is an edge in the graph $G$ and $\mathcal{S}_{i_j}$ 
    is the set of shares for edge $e$ of party $P_{i_j}$. \newline
    
    \textbf{Functionality}: 
    \begin{enumerate}
    \item
      %Upon receiving every inputs from $P_{i_1}, \ldots, P_{i_k}$, 
      $\mathcal{F}_f$ computes $x_{i_j} = \mathsf{Rec}(\secretS{x_{i_j}}_{i_1}, \ldots,  \secretS{x_{i_j}}_{i_k})$ 
      for $j \in [k]$ using the sets $\mathcal{S}_{i_j}$.
    \item $\mathcal{F}_f$ computes $y := f(x_{i_1}, \ldots, x_{i_k})$.
    \item $\mathcal{F}_f$ creates the shares $\secretS{y}_{i_1}, \ldots, \secretS{y}_{i_k} \leftarrow \mathsf{Share}(k, k, y)$.
    \item $\mathcal{F}_f$ sends $\secretS{y}_{i_j}$ to party $P_{i_j}$ for $j \in [k]$.
    \end{enumerate}
  \end{func} 
  \caption{Description of functionality $\mathcal{F}_f$ for computing $f$.}
  \label{fig:f}
\end{figure}

\begin{figure}[ht]
  \begin{func}[Functionality $\mathcal{F}_\text{noise}$]
    
    \textbf{Input}: Functionality $\mathcal{F}_\text{noise}$ receives from all parties $(\epsilon, \delta, s)$ 
    where $(\epsilon, \delta)$ are the DP parameters and $s$ is the sensitivity parameter.\newline
    
    \textbf{Functionality}: 
    \begin{enumerate}
    \item If $\delta = 0$, $\mathcal{F}_\text{noise}$ selects $\eta \sim Lap(0, s/\epsilon)$. 
      Otherwise, $\eta \sim Gauss(0, \frac{2 \ln(1.25/\delta) \cdot (s)^2}{\epsilon^2})$.
    \item $\mathcal{F}_\text{noise}$ creates the shares $\secretS{\eta}_1, \ldots, \secretS{\eta}_n \leftarrow \mathsf{Share}(n, n, \eta)$.
    \item $\mathcal{F}_\text{noise}$ sends $\secretS{\eta}_i$ to party $P_i$ for $i \in [n]$.
    \end{enumerate}
  \end{func}
  \caption{Description of functionality $\mathcal{F}_\text{noise}$ for computing the shared noise.}
  \label{fig:noise}
\end{figure}

\subsection{variance}

	In the following, we derive an upper bound for the variance of $\hat{U}_{f, E}$. 
	% Let us consider $C^n_k$ to be the sampling input space.
	% and let $\mathcal{P}$ be a probability distribution over $C^n_k$.
	Because the variance depends on the sampling method, 
	let us consider the sampling method $\mathsf{BalancedSamp}$ described in Appendix \ref{subsection:algo_sampling}.
	This sampling method produces a regular hypergraph in which each vertex is selected the same amount of times in the hypergraph.
	Consequently, every party appears in at most $\left\lceil \frac{2 |E| }{n} \right\rceil$ edges,
	ensuring that all parties contribute equally to the computation of $\hat{U}_{f, E}$. 

	\begin{restatable}[Variance]{lemma}{lemmavariance}
		\label{lemma:var}
		Assume $f(x, y) \in [0, 1]$ for all $x, y \in \mathbb{X}$. 
		Let $\eta \in \mathbb{R}$ be the noise for some DP mechanism $\mathcal{M}$.
		Using the balanced sampling (Algorithm \ref{algo:sampling}) for sampling the set $E$, 
		the protocol $\prod_\text{U-MPC}$ computes 
		the U-statistic $\hat{U}_{f, E}$ and yields
		\[
			\var(\hat{U}_{f, E}) \leq \frac{ \binom{n}{k} - |E|}{4 |E| \left( \binom{n}{k} - 1 \right)} + \var(\eta).
			% + 2 \frac{k^2 (\Delta f)^2}{n^2 \epsilon^2}
		\]
	\end{restatable}

	\begin{proof}
		This is a genelization of Lemma \ref{lemma:pairwise} in Appendix \ref{section:mse}.
		% The proof follows the same reasoning as in the case $k=2$ which is provided in Lemma \ref{lemma:pairwise}.
		%, Appendix \ref{subsubsection:ours}.
	\end{proof}

	To summarize, we state the following general theorem that is independant from the sampling method.
	Then, we state a proposition for pairwise data, i.e., $k=2$ and $\mathbb{Y} = [0, 1]$ under central $\epsilon$-DP using
	$\mathsf{BalancedSamp}$. 

	\begin{theorem}
		\label{main-thm}
		Let $f: \mathbb{X}^k \to \mathbb{Y}$ be a symmetric function.
		Let $\mathcal{P}$ be a probability distribution over $C^n_k$.
		Let $CC_\text{Noise}$, $CR_\text{Noise}$ be respectively the number of bits exchanged and the number of rounds to generate a shared noise.
		Let $CC_f$, $CR_f$ be respectively the number of bits exchanged and the number of rounds during the online phase for the computation of $f$.
		Let $\mathcal{F}_f$ be the functionality to compute $f$ and $\mathcal{F}_\text{noise}$ the functionality to compute the shared noise.
		The protocol $\prod_\text{U-MPC}$ securely computes the U-statistic $\hat{U}_{f, E}$ under $(\epsilon, \delta)$-DP
		against a semi-honest adversary $\mathcal{A}$ with dishonest majority in the $(\mathcal{F}_f, \mathcal{F}_\text{noise})$-hybrid model.
		It yields
		\begin{equation}
			\var(\hat{U}_{f, E}) = \underset{E \sim \mathcal{P}}{\var} \Big( \frac{1}{|E|} \sum_{v \in E} f(x_v) \Big) + \var(\eta)
		\end{equation}
	where $\eta$ is the noise obtained from an $(\epsilon, \delta)$-DP mechanism $\mathcal{M}$.
	It requires  $O( |E| k^2 \ell + |E| \cdot CC_f + CC_\text{Noise})$ bits of exchange in $O(CR_f + CR_\text{Noise})$ rounds.
	\end{theorem}

	\begin{proof}
		Follows from Lemmas \ref{lemma:correctness}, \ref{lemma:comm}, \ref{lemma:pairwise}.
	\end{proof}

	\begin{restatable}[Pairwise data]{proposition}{pairwise}
		\label{proposition}
		Let $f: \mathbb{X}^2 \to [0, 1]$ be a symmetric function.
		Let $CC_\text{Noise}$, $CR_\text{Noise}$ be respectively the number of bits exchanged and the number of rounds to generate a shared noise.
		Let $CC_f$, $CR_f$ be respectively the number of bits exchanged and the number of rounds during the online phase for the computation of $f$.
		Let $\mathcal{F}_f$ be the functionality to compute $f$ and $\mathcal{F}_\text{noise}$ the functionality to compute the shared noise.
		Using $\mathsf{BalancedSamp}$ (Algorithm \ref{algo:sampling}),
		the protocol $\prod_\text{U-MPC}$ securely computes the U-statistic $\hat{U}_{f, E}$ under $(\epsilon, \delta)$-DP
		against a semi-honest adversary $\mathcal{A}$ with dishonest majority in the $(\mathcal{F}_f, \mathcal{F}_\text{noise})$-hybrid model.
		\begin{equation}
			\begin{split}
			 \var(\hat{U}_{f, E}) &\leq \frac{\binom{n}{2} - |E| }{4 |E| \left( \binom{n}{2} - 1 \right)} + 2 \frac{4 (\Delta f)^2}{n^2 \epsilon^2} \\
			&= O \left(\frac{1}{|E|} + \frac{1}{n^2 \epsilon^2} \right)
 	 		\end{split}	
		\end{equation}		
	where $\eta$ is the noise obtained from an $(\epsilon, \delta)$-DP mechanism $\mathcal{M}$.
	It requires  $O( |E| \cdot (\ell + CC_f) + CC_\text{Noise})$ bits of exchange in $O(CR_f + CR_\text{Noise})$ rounds.
	%and $p = \alpha \comb{n - 1}{k - 1}$ is the expected number of neighbors per party. 
	\end{restatable} 

	\begin{proof}
		Follows from Theorem \ref{main-thm} and Lemma \ref{lemma:pairwise}.
	\end{proof}

	\begin{remark}[Sampling method]
	We make the choice to describe our solution using the algorithm $\mathsf{BalancedSamp}$ for the edges of the 
	hypergraph in proposition \ref{proposition}. 
	The reason for this choice is that it allows to have a regular hypergraph.
	% The reason for this choice is that it allows for simple sampling. 
	% Also, it preserves a balanced structure of the edges on average, i.e., 
	% each party has approximately the same number of neighbors in such a manner that each party contribute the same amount when computing $U_f$. 
	Nevertheless, other sampling methods could be considered. 
	%For instance, using a low-discrepancy graph where the frequency of appearance of elements, pairs, triples, \ldots, $k$-tuples are known. 
	%In this setting, the graph is even more regular than in the sampling with replacement setting.
	For instance, using sample without replacement could be a possibility.
	In \cite{janson1984asymptotic}, the author gives several asymptotic results for the variance of 
	an incomplete U-statistic for different sampling methods, e.g., sampling without replacement, Bernoulli sampling.
    	
	\end{remark}



\section{Comparison{


\newcommand{\GhaziShuffle}{\mathsf{GhaziSM}}
\newcommand{\Ghazi}{\mathsf{Ghazi}}
\newcommand{\Umpc}{\mathsf{Umpc}}
\newcommand{\UmpcTrusted}{\mathsf{UmpcLoc}}
\newcommand{\Bell}{\mathsf{Bell}}

\section{Comparison}
\label{section:comparison}        
In this section, we compare the several approaches under different security settings, 
using various metrics for the computation a U-statistic of degree $k = 2$ under $\epsilon$-DP: 
\begin{itemize}[nosep]
\item $\Ghazi$: non-interactive protocol in \cite{ghazi2024computing}
\item $\GhaziShuffle$: the non-interactive protocol from \cite{ghazi2024computing} in the shuffled model,
  with $r$ servers to shuffle/anonymize messages,
  following the implementation of \citep[Sect.~5]{balle2020private},
\item  $\Bell$: the generic protocol in \cite{bell2020private}
  % \item our protocol $\prod_\text{U-MPC}$ under sampling with replacement for the edges ($\Umpc$) and
  % \item our protocol $\prod_\text{U-MPC}$ under sampling with replacement for the edges
  \janfoot{how about Bell's interactive protocol?}
\item our protocol $\prod_\text{U-MPC}$ under $\mathsf{BalancedSamp}$ (Algorithm \ref{algo:sampling}) for sampling the edges 
  with Protocol \ref{protocol:3} for shared noise ($\Umpc$).
  %  and
  % \item the prior protocol operating under the same assumptions but with local distributed noise generation ($\UmpcTrusted$). 
  % For a detailed argument on why this is possible, see Remark \ref{remark:ldng}. 
\end{itemize}


	\subsection{Mean squared error}
	% Asymptotically, for a U-statistic of degree $k=2$, 
	% our approach $\prod_\text{U-MPC}$ across the two security assumptions ($\Umpc$ and $\UmpcTrusted$) 
	% produces a MSE $O \big( \frac{1}{n^2 \epsilon^2} \big)$. 
	% The protocol $\Bell$ from \cite{bell2020private} results in a MSE $O \big( \frac{1}{\sqrt{n} \epsilon} \big)$
	% while the original protocol from Ghazi et al. \cite{ghazi2024computing} achieves a MSE $O \big( \frac{\mathsf{poly}(\log t)}{n \epsilon^2} \big)$. 
	% The protocol from \cite{ghazi2024computing} augmented by the shuffled model ($\GhaziShuffle$) yields a MSE $ O \big( \frac{\mathsf{poly}(\log t)}{n^2 \epsilon^2} \big)$, 
	% which is comparable to the performance of our protocol, differing only by a factor $\mathsf{poly}(\log t)$.
	% Our approach achieves a lower MSE compared to SOTA solutions.

	Asymptotically, for a U-statistic of degree $k=2$
	and a kernel function $f: \mathbb{X}^2 \to [0,1]$ that is Lipschitz,
	the protocol $\Bell$ from \cite{bell2020private} results in a sample MSE $O \left( \frac{1}{t^2} + \frac{t^2}{n \epsilon^2}\right)$
	while the original protocol from Ghazi et al. \cite{ghazi2024computing} 
	achieves a MSE $O \left( \frac{1}{t^2} + \frac{t^2 \log t}{n \epsilon^2} \right)$. 
	The protocol from \cite{ghazi2024computing} augmented by the shuffled model ($\GhaziShuffle$) yields 
	a MSE $ O \left( \frac{1}{t^2} + \frac{t^2 \log t}{n^2 \epsilon^2} \right)$. 
	Our approach $\prod_\text{U-MPC}$ 
	%across the two security assumptions ($\Umpc$ and $\UmpcTrusted$) 
	produces a MSE $O \left( \frac{1}{|E|} + \frac{1}{n^2 \epsilon^2} \right)$ when sampling with $\mathsf{BalancedSamp}$. 
	%which is comparable to the performance of our protocol, differing only by a factor $\mathsf{poly}(\log t)$.
	%Our approach achieves a lower MSE compared to SOTA solutions.
	For further explanation of the MSEs, please refer to Appendix \ref{section:mse}.
	
	\subsection{Communication cost}
	Let $\ell$ be the number of bits required to represent one element.
	In terms of communication cost, the protocol of Bell et al. \cite{bell2020private} requires to send $O(n \ell t )$ bits in total where $t$ is the number of bins chosen.

	The protocol from Ghazi et al. \cite{ghazi2024computing} allows to reduce the communication cost by requiring that the matrix $A \in \mathbb{R}^{t \times t}$ 
	describing the kernel function is decomposable by two other matrices $L, R \in \mathbb{R}^{d \times t}$ with $d \leq t$. 
	The value $d$ equals $O (\beta^{-2} \log t)$ where $\beta$ is the approximation parameter in the JL theorem. 
	Ghazi et al.'s protocol requires $\beta = 1 / \epsilon \sqrt{n}$, which results in $d = O(\epsilon^2 n \log t)$.
	Hence, $\Ghazi$ requires to send $O(\epsilon^2 n^2 \log t \ell)$ bits in total while
	the shuffled variant $\GhaziShuffle$ requires an additional factor $r$ representing the number servers used for shuffling.
    In \cite{balle2020private}, the authors show that it suffices to take $r = O \left( \log(n) + \kappa \right)$ for $\epsilon$-DP,
	where $\kappa$ is the statistical security parameter,
	yielding $ O \left( (\log(n) + \kappa) n^2 \epsilon^2 (\log t)\ell \right)$ bits in communication cost. 

	For our protocol $\Umpc$, as stated in proposition \ref{proposition},
	the communication cost in the online phase is $ O(|E| \cdot (\ell + CC_f) + CC_\text{Noise})$ bits.
	When the noise is generated according to Protocol $\prod_\text{DLap}$ (Protocol \ref{protocol:3}),
	the communication cost $CC_\text{Noise}$ is at most $O(n^2 \ell)$.
	Consequently, $\Umpc$ requires a total $O( |E| \cdot (\ell + CC_f) + n^2 \ell )$ bits.
	% In the case of local distributed noise generation,
	% $\UmpcTrusted$ requires $ O( |E| \cdot (\ell + CC_f) )$ bits.
		%since the generation of noise is done by the trusted dealer.
		% When the noise is generated according to \cite{eigner2014differentially},
		% the communication cost $CC_\text{Noise}$ is at most $O(n \ell^3)$.
		% Consequently, $\Umpc$ requires a total $O( |E| \cdot (\ell + CC_f) + n \ell^3 )$ bits.

	\subsection{Party computational cost}
	We measure the computational cost as the number of operations performed by each party. 
	In $\Bell$, each party $P_i$ only perturbs its one-hot-vector encoded private data $x_i \in \mathbb{R}^t$,
	which can be done in $ O (t)$ operations. 

	In constrast, the original procotol $\Ghazi$
	requires each party $P_i$ to perform two matrix-vector products between its private vector data $x_i \in \mathbb{R}^t$ and 
	the matrices $L, R \in \mathbb{R}^{d \times t}$.
	\cite{ailon2006approximate} gives a construction for Fast JL Transform which allows to perform the product 
	in $O \left( t \log t + \frac{t \log t}{\beta^2} \right)$ operations by enforcing the sparsity of matrices $L, R$ 
	through preconditioning the projection with a randomized Fourier transform.
	Hence, the $\Ghazi$ algorithm requires $ O \left( \epsilon^2 n t \log t \right)$ operations.
	As for $\GhaziShuffle$, the shuffled model necessitates additional operations to encode each coordinate of the resulting vectors 
	$L x_i, R x_i \in \mathbb{R}^d$, 
	yielding $ O \left( \epsilon^2 n t \log t + t (\kappa + \log n) \right)$ operations 
	where $\kappa$ is the statistical security parameter.

	For our protocol $\Umpc$, let $CC'_f$ denote 
	the computational cost for a single party to evaluate the function $f$ once.
	Assume we use Protocol $\prod_\text{DLap}$ (Protocol \ref{protocol:3}).
	Then, creating distributed Laplace noise requires $O(n)$ overhead per party.
	With balanced sampling, each party $P_i$ participates in $2|E| / n$ edges where $E$ is the set of edges.
	Therefore, in $\Umpc$, the computation per party is $ O \left( |E| \cdot CC'_f / n + n \right)$.
	% For $\UmpcTrusted$, this overhead disappears, giving $ O \left( |E| \cdot CC'_f / n \right) $ operations.

	\subsection{Server computational cost}
	The server computational cost is measured as the number of operations the server has to perform in order to compute the U-statistic.
	In $\Bell$, the server is required to perform $\binom{n}{2}$ matrix-vector products involving $A \in \mathbb{R}^{t \times t}$, 
	which results in $O(n^2 t^2)$ operations. 
	For the original Ghazi et al.'s protocol ($\Ghazi$), a summation of the vectors sent by the parties is required, 
	resulting in $n \cdot d$ operations. 
	Furthermore, a dot product between vectors of size $d = O(\epsilon^2 n \log t)$ is required. 
	Hence, it requires $ O(\epsilon^2 n^2 \log t + \epsilon^2 n \log t) = O\left( (\epsilon n)^2 \log t \right)$ operations. 
	For $\GhaziShuffle$, it requires $O \left( (\kappa + \log n) \epsilon^2 n^2 \log t \right)$ operations to the server.

	%For our protocol ($\Umpc$ and $\UmpcTrusted$), it only requires $n$ additions. 
	For our protocol $\Umpc$, it only requires $n$ additions. 

	\subsection{Summary}

	We summarize the comparison results in Table \ref{tab1}.
	For each metric in Table \ref{tab1}, we suppress the asymptotic notation.
	The communication cost is measured as the total number of bits exchanged during the protocol.
	The computational cost is the number of operations done by either the server or one party.

	Recall that $n$ represents the number of parties and $t$ denotes the number of discretization bins.
	The value $\epsilon$ is the DP parameter. 
	$\ell$ is the number of bits required to represent one element.
	% Let $d = O(\epsilon^2 n \log t)$ be the reduced dimension when using the JL theorem.
	The set $E$ represents the set of edges selected for the graph $G$ in our protocol $\prod_\text{U-MPC}$.
	% The parameter $\kappa$ is the statistical security parameter when implementing the shuffled model.
	% The value $p = \underset{i \in [n]}{\esp}[ | E_{ \{ i \}} |]$ is the expected number of neighbors per party in the protocol $\prod_\text{U-MPC}$.
	The term $CC_f$ represents the communication cost incurred during the online phase of the evaluation of $f$ in $\prod_\text{U-MPC}$.
	while $CC'_f$ represents
	the computational cost per party incurred during the online phase of the evaluation of $f$ in Protocol $\prod_\text{U-MPC}$.

\begin{table*}[t]
  \centering
  \caption{Protocol comparison}
  \label{tab1}
  \begin{tabular}{cccccc}
    \Xhline{2\arrayrulewidth}
    \noalign{\vskip 2mm}
    \textbf{Protocol} & \textbf{MSE}${(1)}$ & \textbf{Total online comm. cost}$^{(2)}$ & \textbf{Party computation cost}$^{(3)}$ & \textbf{Server computation cost}$^{(4)}$ \\
    \noalign{\vskip 2mm}
    \Xhline{2\arrayrulewidth}
    \rule{0pt}{4ex}$\Bell$ \cite{bell2020private} & $\frac{1}{t^2} + \frac{t^2}{n \epsilon^2}$ & $n \ell t $ & $t$ &  $n^2 t^2$ \\
    \noalign{\vskip 2mm}
    \hline
    
    \rule{0pt}{4ex}$\Ghazi$ \cite{ghazi2024computing} & $\frac{1}{t^2} + \frac{t^2 \log t}{\epsilon^2 n}$ & $ n^2 \epsilon^2 (\log t)\ell$ 
    & $\epsilon^2 n t \log t$ &  $\epsilon^2 n^2 \log t$\\
    
    \rule{0pt}{5ex}$\GhaziShuffle$ \cite{ghazi2024computing} & $\frac{1}{t^2} + \frac{ t^2 \log t}{\epsilon^2 n^2} $ & $ (\log n) n^2 \epsilon^2 (\log t)\ell $ 
    & $ \epsilon^2 n t \log t  + t \log n$ 
    & $ (\log n) \epsilon^2 n^2 \log t$ \\
    
    \noalign{\vskip 2mm}
    \hline
    
    \rule{0pt}{5ex} \makecell{$\Umpc$ \\(Prot. \ref{protocol})} & $\frac{1}{|E|} + \frac{1}{n^2 \epsilon^2}$ & $ |E| \cdot (\ell + CC_f) + n^2 \ell $ & $ \frac{|E|}{n} \cdot CC'_f + n$ & $n$ \\
    
    % \rule{0pt}{5ex} \makecell{$\UmpcTrusted$ \\ (Prot. \ref{protocol})} & $\frac{1}{|E|} + \frac{1}{n^2 \epsilon^2}$ & $ |E| \cdot (\ell + CC_f)$ &  $ \frac{|E|}{n} \cdot CC'_f$ & $n$ \\	
    \noalign{\vskip 2mm}
    \Xhline{2\arrayrulewidth}
  \end{tabular}
  
  \vspace{0.3cm}
  
  For readability, asymptotic notations are suppressed.\\
  $^{(1)}$MSE computed between the estimator and the sampled U-statistic.\\
  $^{(2)}$The total communication cost is measured in total bits exchanged in the online phase. \\
  $^{(3)}$Party computational cost is measured in number of operations per party. \\
  $^{(4)}$Server computational cost is measured in the number of operations.
\end{table*}

% \quentinadd{
% We observe that our protocol $\prod_\text{U-MPC}$ achieves lower MSE than the other protocols. 
% Among the alternatives, only $\mathsf{Ghazi\text{-}TD}$ approaches the MSE attainable in the central-DP setting. 
% With the assistance of a trusted dealer, 
% our protocol ($\mathsf{UMPC - TD}$) requires $O(n p \ell + \alpha n^2 CC_f)$ bits of communication, 
% which is comparable to the $O(r n \ell d)$ bits required by $\mathsf{Ghazi - TD}$.
% Indeed, when $CC_f = \mathsf{poly}(\ell)$ remains small and since $\alpha \in [0, 1]$, 
% the communication complexity of $\UmpcTrusted$ is dominated by $O(\alpha n^2 \mathsf{poly}(\ell))$, 
% which can be favorable compared to the linear dependence $O(r n \ell d)$ of $\mathsf{Ghazi - TD}$, especially for large $n$. 
% In terms of computation cost, when $CC'_f$ is small compared to $d = O(e^{-2} \log t)$, i.e., $CC'_f \ll d$, the setup $\mathsf{UMPC - TD}$ is faster.
% }


        


\appendix



\section{Drawing distributed noise}
\label{section:drawing_noise}
	
When generating shared noise from Laplace or Gaussian distribution, there are among others the following two possibilities:
\begin{enumerate}
\item sample a noise $x$ from continuous distribution, e.g., Laplace distribution $\text{Lap}(\mu, b)$, 
  then, using our fixed-precision representation of numbers, 
  convert this into $\mathbb{F}_{2^\ell}$ using the $\mathsf{int}^{-1}$ and $\mathsf{convert}$ mappings (see Appendix \ref{app:data_representation}). 
\item Another option would be to directly draw a noise $x'$ from a discrete distribution, e.g.,
  discrete Laplace distribution noted $\text{DLap}(\mu, a)$ where $a$ is the scale parameter (see \cite{canonne2020discrete, eigner2014differentially}). 
\end{enumerate}
Those two approaches are at the end equivalent 
when one is in the distributed setting (manipulating values in $\mathbb{F}_{2^\ell}$). 
% However, we choose the first approach as there are more techniques to sample in the literature compared to the discrete sampling.
	In the following, we describe approaches to sample from (discrete) Laplace distribution and Gaussian distribution.




\subsubsection{The Distributed Polar Box-Muller Method}
\paragraph{Threat model and functionality}
As in the main protocol $\prod_\text{U-MPC}$, we place ourselves in the same setup. 
We assume a static semi-honest adversary $\mathcal{A}$ in the dishonest majority setting.
To compute the distributive $\mod$, we refer to the functionality $\mathcal{F}_\text{mod}$ described in Figure \ref{functionality:mod}.

\begin{figure}[h!]
  \begin{func}[Functionality $\mathcal{F}_\text{mod}$]
    \textbf{Input}: Functionality $\mathcal{F}_\text{mod}$ receives $\secretS{x}_i$ 
    from party $P_{i}$ for all $i \in [n]$ and a public value $m$. \newline
    
    
    \textbf{Functionality}: 
    \begin{enumerate}
    \item $\mathcal{F}_\text{mod}$ computes $x = \mathsf{Rec}(\secretS{x}_{1}, \ldots,  \secretS{x}_{n})$.
    \item $\mathcal{F}_\text{mod}$ computes $y := x \mod m$.
    \item $\mathcal{F}_\text{mod}$ creates the shares $\secretS{y}_1, \ldots, \secretS{y}_n \leftarrow \mathsf{Share}(n, n, y)$.
    \item $\mathcal{F}_\text{mod}$ sends $\secretS{y}_i$ to party $P_i$ for $i \in [n]$.
    \end{enumerate}
  \end{func} 
  \caption{Description of functionality $\mathcal{F}_\text{mod}$ for computing $\mod$.}
  \label{functionality:mod}
\end{figure}

